On the security of key distribution based on Johnson-Nyquist noise

We point out that arguments for the security of Kish's noise-based cryptographic protocol have relied on an unphysical no-wave limit, which if taken seriously would prevent any correlation from developing between the users. We introduce a noiseless version of the protocol, also having illusory security in the no-wave limit, to show that noise and thermodynamics play no essential role. Then we prove generally that classical electromagnetic protocols cannot establish a secret key between two parties separated by a spacetime region perfectly monitored by an eavesdropper. We note that the original protocol of Kish is vulnerable to passive time-correlation attacks even in the quasi-static limit. Finally we show that protocols of this type can be secure in practice against an eavesdropper with noisy monitoring equipment. In this case the security is a straightforward consequence of Maurer and Wolf's discovery that key can be distilled by public discussion from correlated random variables in a wide range of situations where the eavesdropper's noise is at least partly independent from the users' noise.

==> riedelheader.tex <==
% ***********************************************************
% ******************* PHYSICS HEADER ************************
% ***********************************************************
% Version 2
% Modification by C. Jess Riedel

%The following tries to let TeXShop know to use a custom macro engine:
%!TEX TSprogram = TeXify 

\usepackage{
	amssymb, % Math symbols such as \mathbb
	amsthm, % Theorem Formatting
	graphicx, % Allows for eps images
	xspace,
	overpic,
	ifthen,
	verbatim, 
	subfigure, % allows figure sub parts [ (a), (b), etc.]
         %subfig, % new version of subfigure
	appendix,
	ifthen,
	nicefrac, %for simple inline fractions
	%afterpage, %allows the \afterpage{clearpage} command
	%placeins, %allows the \Floatbarrier command
	%multicol, % Allows for multiple columns
	color, % Change text and page color
	tensor, %for pre-posed subscript and superscripts, as well as GR-like spacing
	etoolbox, %for robust if/then control
	centernot, %for negating \ll and \gg, and other stuff
	%stfloats, %This doesn't seem to work.  %A bad point of the starred environments {figure*} and {table*} (which create floats which span the whole page instead of a column) is that they can be placed only at the top of the page or on their own page. If you try to specify their position using modifiers like b or h they will be ignored. Add \usepackage{stfloats} to the preamble in order to alleviate this problem with regard to placing these floats at the bottom of a page, using the optional specifier [b]. Default is [tbp]. However, h still does not work.
	%fixltx2e, %Prevent "starred" (page spanning) figures from being placed out-of-order with respect to their "non-starred" (column spanning) counterparts.
	MnSymbol, %for \rrangle and \llangle
	amsmath,
	bm
} 

% Alter some LaTeX defaults for better treatment of figures.
% Source: http://mintaka.sdsu.edu/GF/bibliog/latex/floats.html
% See p.105 of "TeX Unbound" for suggested values.
% See pp. 199-200 of Lamport's "LaTeX" book for details.
%   General parameters, for ALL pages:
\renewcommand{\topfraction}{0.9}	% max fraction of floats at top
\renewcommand{\bottomfraction}{0.8}	% max fraction of floats at bottom
%   Parameters for TEXT pages (not float pages):
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}     % 2 may work better
\setcounter{dbltopnumber}{2}    % for 2-column pages
\renewcommand{\dbltopfraction}{0.9}	% fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}	% allow minimal text w. figs
%   Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.7}	% require fuller float pages
% N.B.: floatpagefraction MUST be less than topfraction !!
\renewcommand{\dblfloatpagefraction}{0.7}	% require fuller float pages
% remember to use [htp] or [htpb] for placement


 
% Bra-ket notation
%---
%Note that dealing with \mvert \vert \lvert \rvert \mid and | is tricky.  Using \vert seems to work except for kets and bras involving arrows like \uparrow, in which case the spacing is bad.  \lvert and \rvert fix this.  But if you use them, you need to use \mvert in matrix elements; otherwise elements involving arrows will look kinda weird.  but this make other matrixelements *really* weird, so we don't do this.  the stuff below is an imperfect compromise.  consider revising in the future.

%\newcommand{\bra}[1]{\langle #1 \vert  }
%\newcommand{\ket}[1]{\vert #1 \rangle  }
%\newcommand{\Bra}[1]{\left\langle #1 \right\vert  }
%\newcommand{\Ket}[1]{\left\vert #1 \right\rangle  }
\newcommand{\bra}[1]{\langle #1 \rvert  }
\newcommand{\ket}[1]{\lvert #1 \rangle  }
\newcommand{\Bra}[1]{\left\langle #1 \right\rvert  }
\newcommand{\Ket}[1]{\left\lvert #1 \right\rangle  }

%\newcommand{\braket}[2]{  \langle #1 \mvert #2 \rangle  }
%\newcommand{\Braket}[2]{  \left\langle #1 \middle\mvert #2 \right\rangle  }
%\newcommand{\matrixelement}[3]{  \langle #1 \mvert #2 \mvert #3\rangle  }
%\newcommand{\Matrixelement}[3]{  \left\langle #1 \middle\mvert #2 \middle\mvert #3 \right\rangle  }
\newcommand{\braket}[2]{  \langle #1 \vert #2 \rangle  }
\newcommand{\Braket}[2]{  \left\langle #1 \middle\vert #2 \right\rangle  }
\newcommand{\matrixelement}[3]{  \langle #1 \vert #2 \vert #3\rangle  }
\newcommand{\Matrixelement}[3]{  \left\langle #1 \middle\vert #2 \middle\vert #3 \right\rangle  }

\newcommand{\ketbra}[2]{  \lvert #1 \rangle \langle #2 \rvert }
\newcommand{\Ketbra}[2]{  \left\lvert #1 \middle\rangle \middle\langle #2 \right\rvert }
\newcommand{\projector}[1]{  \lvert #1 \rangle \langle #1 \rvert }
\newcommand{\Projector}[1]{  \left\lvert #1 \middle\rangle \middle\langle #1 \right\rvert }

% Average and abs notation  
%THIS SHOULD BE REPLACED WITH TECHNIQUES FROM HERE:
% http://tex.stackexchange.com/questions/43008/absolute-value-symbols
\newcommand{\abs}[1]{| #1 |} % for absolute value
\newcommand{\Abs}[1]{\left| #1 \right|}
\newcommand{\aabs}[1]{|| #1 ||} % for double absolute value, like a matrix norm
\newcommand{\AAbs}[1]{\left| \left| #1 \right| \right|}
\newcommand{\avg}[1]{\langle #1 \rangle} % for average
\newcommand{\Avg}[1]{\left\langle #1 \right\rangle}
%\newcommand{\aavg}[1]{\lAngle #1 \rAngle} % for double-line average
%\newcommand{\AAvg}[1]{\left\lAngle #1 \right\rAngle}
\newcommand{\aavg}[1]{\llangle #1 \rrangle} % for double-line average
\newcommand{\AAvg}[1]{\left\llangle #1 \right\rrangle}



% Derivative notation
\newcommand{\dd}{\,\mathrm{d}} % differential d
\newcommand{\fd}[2]{\frac{\d #1}{\d #2}} % for full derivatives
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}} % for partial derivatives
\newcommand{\pdc}[3]{\left( \frac{\partial #1}{\partial #2} \right)_{#3}} % for thermodynamic partial derivatives

% Decoherence Symbols
\newcommand{\MI}{\ensuremath{\mathcal{I}}}
\newcommand{\Sys}{\ensuremath{\mathcal{S}}}
\newcommand{\Env}{\ensuremath{\mathcal{E}}}
\newcommand{\Frag}{\ensuremath{\mathcal{F}}}
\newcommand{\FragBar}{{\ensuremath{{\overline{\mathcal{F}}}}}}
\newcommand{\Obs}{\ensuremath{\mathcal{O}}}
\newcommand{\Aux}{\ensuremath{\mathcal{R}}}
\newcommand{\Glob}{\ensuremath{\mathcal{H}}}
\newcommand{\sharpof}[1]{\ensuremath{\tensor[^\sharp]{#1}{}}}

\newcommand{\mcA}{\ensuremath{\mathcal{A}}}
\newcommand{\mcB}{\ensuremath{\mathcal{B}}}
\newcommand{\mcC}{\ensuremath{\mathcal{C}}}

% Brackets
%\newcommand{\p}{\ensuremath{\left}}
%\newcommand{\q}{\ensuremath{\right}}

% Roman Operators  %not compatible with IOP
% Template:    \DeclareMathOperator{\Sample}{Sample}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\arctanh}{arctanh}
%\DeclareMathOperator{\coth}{coth}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\csch}{csch}

% Cross references
\newcommand{\refstyle}{2}  
% refstyle=1 for capitalized-appreviated (Eq., Fig., etc.)
% refstyle=2 for lowercase-full (equation, figure, etc.) 
\newcommand{\eqrefstyle}{2}  
% eqrefstyle=1 for always leaving out 'equation' 
% eqrefstyle=2 for having it optionally for emphasis
% eqrefstyle=3 for always having 'equation' 
% For the beginning of a sentence, you should spell out the capitalized work (Figure, Equation, etc.) explicitly 
% without any commands, because that's how it will appear in any style.
% If you want to add a third style, see here: http://tex.stackexchange.com/questions/29905/how-to-form-if-or-then-conditionals-in-tex
\newcommand{\Jeqref}[1] {\ifnum\refstyle=1{Eq.~(\ref{#1})}\else{equation (\ref{#1})}\fi}
% This is a helper command for putting 'Eq.' or 'equation' 
\newcommand{\Jeqsref}[1] {\ifnum\refstyle=1{Eqs.~(\ref{#1})}\else{equations (\ref{#1})}\fi}
% For multiple equations, the all but the first number are added explicitly by the user using \eqref  .  For example...
% ...by examining \Eqsrefs{ref1}, \eqref{ref2}, and \eqref{3}, we can see that....
\newcommand{\EQref}[1] {\ifnum\eqrefstyle=1{(\ref{#1})}\else{\Jeqref{#1}}\fi}
\newcommand{\EQsref}[1] {\ifnum\eqrefstyle=1{(\ref{#1})}\else{\Jeqsref{#1}}\fi}
% The above two commands try to include 'equation' or 'Eq.', for emphasis, when allowed.
\newcommand{\Eqref}[1]  {\ifnum\eqrefstyle=3{\Jeqref{#1}}\else{(\ref{#1})}\fi}
\newcommand{\Eqsref}[1]  {\ifnum\eqrefstyle=3{\Jeqsref{#1}}\else{(\ref{#1})}\fi}
% the above two commands try to suppress 'equation' or 'Eq.', for emphasis, when allowed.  These are the mostly commonly used commands.
% Note that APS style is to keep the equation number in parentheses even if writing 'Equation' before 
% it, which happens at the beginning of a sentence.
% In all of the above, I use \ref instead of \eqref (which automatically includes parentheses)  so the code is 
% transparent, and doesn't rely on amsmath
\newcommand{\Figref}[1]{\ifnum\refstyle=1{Fig.~\ref{#1}}\else{figure~\ref{#1}}\fi}
\newcommand{\Figsref}[1]{\ifnum\refstyle=1{Figs.~\ref{#1}}\else{figures~\ref{#1}}\fi}
\newcommand{\Appref}[1]{\ifnum\refstyle=1{App.~\ref{#1}}\else{appendix~\ref{#1}}\fi}
\newcommand{\Appsref}[1]{\ifnum\refstyle=1{Apps.~\ref{#1}}\else{appendices~\ref{#1}}\fi}
\newcommand{\Chref}[1]{\ifnum\refstyle=1{Ch.~\ref{#1}}\else{chapter~\ref{#1}}\fi}
\newcommand{\Chsref}[1]{\ifnum\refstyle=1{Chs.~\ref{#1}}\else{chapters~\ref{#1}}\fi}
\newcommand{\Secref}[1]{\ifnum\refstyle=1{Sec.~\ref{#1}}\else{section~\ref{#1}}\fi}
\newcommand{\Secsref}[1]{\ifnum\refstyle=1{Secs.~\ref{#1}}\else{sections~\ref{#1}}\fi}
\newcommand{\Refref}[1]{\ifnum\refstyle=1{Ref.~\cite{#1}}\else{reference~\cite{#1}}\fi}
\newcommand{\Refsref}[1]{\ifnum\refstyle=1{Refs.~\cite{#1}}\else{references~\cite{#1}}\fi}
%use this when referring to a reference as part of the sentence
\newcommand{\Itref}[1]{\#\ref{#1}}


% Editing colors
\newcommand{\draftmode}{1}    %to control draft colors below
\newcommand{\notetoself}[1]{\ifnum \draftmode=1 {\color[rgb]{0,0,0.8} [#1]} \fi}  %notes to self in blue when \draftmode==1.  invisible otherwise
\newcommand{\cuttext}[1]{\ifnum \draftmode=1 {\color[rgb]{0,0.5,0} [#1]} \fi}  %cut out text in green when \draftmode==1.  invisible otherwise
\newcommand{\warntext}[1]{{\ifnum \draftmode=1 \color[rgb]{0.9,0.6,0} \else  \color{black} \fi} #1}  
      %warning text in orange when \draftmode==1.  regular black otherwise
%\newcommand{\siren}[1]{{\ifnum \draftmode=1 \color[rgb]{0.9,0.6,0} \else  \color{black} \fi} [#1]}  
\newcommand{\siren}[1]{{\color[rgb]{0.8,0.0,0} [#1]}}  %for loud error-type text that prints red *always*
%\newcommand{\newtext}{\color{black}} %this is deprecated
%\newcommand{\oldtext}{\ifnum \draftmode=1 \color[gray]{0.5} \else \color{black} \fi}  % deprecated version
%\newcommand{\oldtext}{\ifthenelse{\equal{\draftmode}{1}}{\color[gray]{0.5}}{\color{black}}}

%Other
\newcommand{\etal}{et~al.\ }

%\def\FCW{0.98\columnwidth}
%\def\HPW{0.48\textwidth}
%\def\TQPW{0.73\textwidth}
%\def\FPW{0.98\textwidth}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      Notes on mathematical equation environments         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%    "The eqnarray and eqnarray* environments...are not recommended because they produce 
%    inconsistent spacing of the equal signs and make no attempt to prevent overprinting of the 
%    equation body and equation number."   -Short Math Guide, AMS

%    Apparently, the align environment (from the amsmath package) can always be used, whether 
%    multi-line or not, in place of the equation environment

%    Also usable are the environments:
%    --------------------------------------------------------------------------------------------------------------------------- 
%      multiline             puts single eq number on last line of multi-line object.  Also, doesn't let you 
%                                   manually align each line, like aligning the equal signs. Instead it only lets 
%                                  you push everything left or right.
%      gather                 exactly like align, with each line of multi-line object numbered individually, 
%                                  except that gather centers all eqns rather than aligns the ='s.  Doesn't 
%                                  accept &'s.
%      flalign*               collects several small equations near sides. the "*" means it has no 
%                                  numbering.  see Short Math Guide, AMS)

%   In addition, there are mathematical sub-environments, which can only appear inside one of 
%   the regular environments just listed:
%    --------------------------------------------------------------------------------------------------------------------------- 
%      split                    forces any outer environment to treat a multi-line object as a single line for 
%                                  numbering purposes, yielding a vertically centered eqn number for the object
%      aligned              Similar to 'split'.  So far, I have only seen places where they are equivalent (up 
%                                  to a *very* slight spacing difference) or split is superior
%      subequations   wrapped around any of the above environments, it forces "sub numbering":   
%                                  3a, 3b, etc.  Properly placed labels can be referenced as (3) or (3b).

%   Nesting a split environment inside your existing align environment seems to do everything 
%   that align does except to give it a single number:
%\begin{align}\begin{split}
%...
%\end{split}\end{align}

%   Aligned is supposed to work just like align except that it's designed to go inside other 
%   environments.  This seems to make it do the same thing as split
%\begin{align}\begin{aligned}
%...
%\end{aligned}\end{align}

%   The one place where I have observed a difference between split and aligned is if I want 
%   multiple equations (with their own number), but only some of them extend onto multiple lines.  
%   In this case, split seems to work but aligned breaks.
%   This works:
%\begin{align}
%\begin{split}F(x) &= \mathrm{first part of RHS} \\  & \qquad + \mathrm{second part of RHS}  \end{split} \\
%G(x) &= \mathrm{another RHS} , \\
%H(x) &= \mathrm{yet another RHS}.
%\end{align}
%   but this does not (it has alignment issues)
%\begin{align}
%\begin{aligned}F(x) &= \mathrm{first part of RHS} \\  & \qquad + \mathrm{second part of RHS}  \end{aligned} \\
%G(x) &= \mathrm{another RHS} , \\
%H(x) &= \mathrm{yet another RHS}.
%\end{align}
%   Presumably, aligned has uses for creating weirdly blocked or spaced equations, but I just haven't been introduced to them.

%   Apparently, trying to create a nice alias like
%\newcommand{\balin}{\begin{align}\begin{aligned}}
%   is doomed to failure because the AMS align environment is tricky/obnoxious


% ***********************************************************
% ********************** END HEADER *************************
% ***********************************************************
